Tunable Hybrid Proposal Networks for the Open World

Current state-of-the-art object proposal networks are trained with a closed-world assumption, meaning they learn to only detect objects of the training classes. These models fail to provide high recall in open-world environments where important novel objects may be encountered. While a handful of recent works attempt to tackle this problem, they fail to consider that the optimal behavior of a proposal network can vary significantly depending on the data and application. Our goal is to provide a flexible proposal solution that can be easily tuned to suit a variety of open-world settings. To this end, we design a Tunable Hybrid Proposal Network (THPN) that leverages an adjustable hybrid architecture, a novel self-training procedure, and dynamic loss components to optimize the tradeoff between known and unknown object detection performance. To thoroughly evaluate our method, we devise several new challenges which invoke varying degrees of label bias by altering known class diversity and label count. We find that in every task, THPN easily outperforms existing baselines (e.g., RPN, OLN). Our method is also highly data efficient, surpassing baseline recall with a fraction of the labeled data.

==> tables/tl10_ships_challenge_full.tex <==
\begin{table*}[t]
\centering
\resizebox{.95\linewidth}{!}{


\begin{tabular}{llc|cccc|cccc|cccc}
\toprule
                          &                                      & Images /    & \multicolumn{4}{c|}{OOD}                                      & \multicolumn{4}{c|}{ID}                                       & \multicolumn{4}{c}{ALL}                                       \\
Split                     & Model                                & Instances   & AUC           & AR10          & AR100         & AR1k          & AUC           & AR10          & AR100         & AR1k          & AUC           & AR10          & AR100         & AR1k          \\ \hline\hline \noalign{\vskip .6mm}
\multirow{6}{*}{Military}  & Faster R-CNN                         & 1.5k / 4.7k & 11.8          & 11.8          & 12.2          & 24.3          & 65.6          & 75.6          & 79.4          & 81.3          & 33.3          & 37.1          & 39.1          & 47.1          \\
                          & OLN                                  & 1.5k / 4.7k & 23.0          & 23.4          & 28.1          & 35.8          & 69.0          & 79.2          & 84.4          & 85.4          & 41.3          & 45.2          & 50.6          & 55.6          \\ \cdashline{2-15} \noalign{\vskip .6mm}
                          & STPN ($\lambda_{CLS}=0$) & 1.5k / 6.1k & \textbf{26.7} & \textbf{27.1} & \textbf{33.7} & \textbf{37.8} & 69.2          & 79.2          & 84.6          & 85.4          & 43.6 & 47.5 & 54.1 & 56.9 \\
                          & STPN ($\lambda_{CLS}=0.10$)       & 1.5k / 6.1k & 26.6          & 27.0          & 33.6          & 37.8          & 69.3 & 79.4          & 84.7 & 85.4 & 43.6          & 47.5          & 54.1          & 56.9          \\
                          & \textbf{STPN ($\boldsymbol{\lambda_{CLS}=0.25}$)}       & 1.5k / 6.1k & 26.6          & 27.0          & 33.7          & 37.8          & 69.4          & 79.8 & 84.8          & 85.4          & \textbf{43.6}          & \textbf{47.6}          & \textbf{54.2}          & \textbf{56.9}          \\
                          & STPN ($\lambda_{CLS}=0.50$)       & 1.5k / 6.1k & 26.5          & 26.6          & 33.7          & 37.8          & \textbf{69.5}          & \textbf{79.8}          & \textbf{84.8}          & \textbf{85.4}          & 43.6          & 47.3          & 54.2          & 56.9          \\ \hline
\multirow{6}{*}{Civilian} & Faster R-CNN                         & 1.0k / 4.4k & 16.0          & 16.8          & 17.8          & 29.1          & 33.4          & 29.5          & 44.3          & 51.2          & 24.6          & 22.6          & 31.0          & 40.1          \\
                          & OLN                                  & 1.0k / 4.4k & 38.7          & 38.4          & 49.2          & 56.6          & 35.6          & 30.7          & 47.9          & 54.3          & 36.9          & 33.8          & 48.5          & 55.5          \\ \cdashline{2-15} \noalign{\vskip .6mm}
                          & STPN ($\lambda_{CLS}=0$) & 1.0k / 5.7k & 46.1 & 46.6 & 58.3 & 64.2 & 36.2 & 31.0          & 48.3 & 54.9 & 40.8 & 37.8 & 53.3 & 59.5 \\
                          & \textbf{STPN ($\boldsymbol{\lambda_{CLS}=0.10}$)}       & 1.0k / 5.7k & \textbf{46.3}          & \textbf{47.2}          & \textbf{58.4}          & \textbf{64.2}          & \textbf{36.4}          & 31.4          & \textbf{48.5}          & 55.0          & \textbf{41.0}          & \textbf{38.2}          & \textbf{53.4}          & \textbf{59.6}          \\
                          & STPN ($\lambda_{CLS}=0.25$)       & 1.0k / 5.7k & 46.2          & 47.1          & 58.5          & 64.1          & 36.4          & 31.4          & 48.4          & 54.9          & 41.0          & 38.2          & 53.4          & 59.5          \\
                          & STPN ($\lambda_{CLS}=0.50$)       & 1.0k / 5.7k & 46.2          & 46.9          & 58.3          & 64.1          & 36.3          & \textbf{31.5}          & 48.3          & \textbf{55.1}          & 41.0          & 38.2          & 53.3          & 59.6       
                        \\
\bottomrule
\end{tabular}


}
\vspace{-2mm}
\caption{Full results on the \textit{ships} challenge when using a model trained with $\lambda_{CLS}=0.10$. The listed $\lambda_{CLS}$ in the table is the value used during inference-time.}
\label{tab:tl10_ships_challenge_full}
%\vspace{-3mm}
\end{table*}
